LOSDD: Leave-Out Support Vector Data Description for Outlier Detection

Support Vector Machines have been successfully used for one-class classification (OCSVM, SVDD) when trained on clean data, but they work much worse on dirty data: outliers present in the training data tend to become support vectors, and are hence considered "normal". In this article, we improve the effectiveness to detect outliers in dirty training data with a leave-out strategy: by temporarily omitting one candidate at a time, this point can be judged using the remaining data only. We show that this is more effective at scoring the outlierness of points than using the slack term of existing SVM-based approaches. Identified outliers can then be removed from the data, such that outliers hidden by other outliers can be identified, to reduce the problem of masking. Naively, this approach would require training N individual SVMs (and training $O(N^2)$ SVMs when iteratively removing the worst outliers one at a time), which is prohibitively expensive. We will discuss that only support vectors need to be considered in each step and that by reusing SVM parameters and weights, this incremental retraining can be accelerated substantially. By removing candidates in batches, we can further improve the processing time, although it obviously remains more costly than training a single SVM.

==> results.tex <==
\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{Annthyroid\_02}} & \multicolumn{2}{l}{\rot{Annthyroid\_05}} & \multicolumn{2}{l}{\rot{Arrhythmia\_02}} & \multicolumn{2}{l}{\rot{Arrhythmia\_05}} & \multicolumn{2}{l}{\rot{Arrhythmia\_10}} & \multicolumn{2}{l}{\rot{Arrhythmia\_20}} & \multicolumn{2}{l}{\rot{Cardiotocography\_02}} & \multicolumn{2}{l}{\rot{Cardiotocography\_05}} & \multicolumn{2}{l}{\rot{Cardiotocography\_10}} & \multicolumn{2}{l}{\rot{Cardiotocography\_20}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &                mean &    std &                mean &    std &                mean &    std &                mean &    std \\
\hline
KNN            &  \textbf{0.703} &  0.018 &  \textbf{0.673} &  0.008 &           0.772 &  0.090 &           0.793 &  0.053 &           0.782 &  0.027 &           0.759 &  0.035 &               0.763 &  0.059 &               0.701 &  0.024 &               0.611 &  0.017 &               0.498 &  0.009 \\
LOSEVM\_1       &           0.516 &  0.022 &           0.498 &  0.011 &  \textbf{0.817} &  0.079 &  \textbf{0.831} &  0.055 &  \textbf{0.834} &  0.028 &  \textbf{0.797} &  0.038 &               0.796 &  0.035 &               0.772 &  0.022 &                0.75 &  0.030 &               0.717 &  0.061 \\
LOSEVM\_5       &           0.516 &  0.022 &           0.498 &  0.011 &           0.815 &  0.080 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &                0.81 &  0.036 &               0.786 &  0.016 &               0.761 &  0.017 &      \textbf{0.745} &  0.007 \\
LOSEVM\_10      &           0.516 &  0.022 &           0.498 &  0.011 &           0.815 &  0.080 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &               0.817 &  0.038 &                0.79 &  0.017 &               0.765 &  0.019 &      \textbf{0.745} &  0.005 \\
LOSEVM\_20      &           0.516 &  0.022 &           0.498 &  0.011 &           0.814 &  0.081 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &               0.817 &  0.037 &      \textbf{0.791} &  0.017 &      \textbf{0.766} &  0.019 &      \textbf{0.745} &  0.004 \\
LOSEVM\_SVDD\_1  &           0.516 &  0.022 &           0.498 &  0.011 &  \textbf{0.817} &  0.079 &  \textbf{0.831} &  0.055 &  \textbf{0.834} &  0.028 &  \textbf{0.797} &  0.038 &               0.794 &  0.036 &               0.771 &  0.023 &               0.748 &  0.032 &               0.716 &  0.056 \\
LOSEVM\_SVDD\_5  &           0.516 &  0.022 &           0.498 &  0.011 &           0.815 &  0.080 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &                0.81 &  0.033 &               0.783 &  0.015 &               0.762 &  0.019 &               0.744 &  0.007 \\
LOSEVM\_SVDD\_10 &           0.516 &  0.022 &           0.498 &  0.011 &           0.815 &  0.080 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &      \textbf{0.819} &  0.038 &                0.79 &  0.018 &               0.765 &  0.019 &      \textbf{0.745} &  0.005 \\
LOSEVM\_SVDD\_20 &           0.516 &  0.022 &           0.498 &  0.011 &           0.814 &  0.081 &           0.829 &  0.056 &           0.833 &  0.028 &  \textbf{0.797} &  0.038 &      \textbf{0.819} &  0.038 &                0.79 &  0.018 &      \textbf{0.766} &  0.019 &      \textbf{0.745} &  0.005 \\
OCSVM          &           0.516 &  0.022 &           0.498 &  0.011 &            0.69 &  0.068 &           0.712 &  0.037 &           0.667 &  0.056 &           0.665 &  0.029 &               0.811 &  0.033 &               0.788 &  0.018 &               0.763 &  0.019 &               0.744 &  0.004 \\
SVDD           &           0.516 &  0.022 &           0.498 &  0.011 &            0.69 &  0.068 &           0.712 &  0.037 &           0.667 &  0.056 &           0.665 &  0.029 &               0.811 &  0.033 &               0.788 &  0.018 &               0.763 &  0.019 &               0.744 &  0.004 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{HeartDisease\_02}} & \multicolumn{2}{l}{\rot{HeartDisease\_05}} & \multicolumn{2}{l}{\rot{HeartDisease\_10}} & \multicolumn{2}{l}{\rot{HeartDisease\_20}} & \multicolumn{2}{l}{\rot{Hepatitis\_05}} & \multicolumn{2}{l}{\rot{Hepatitis\_10}} & \multicolumn{2}{l}{\rot{InternetAds\_02}} & \multicolumn{2}{l}{\rot{InternetAds\_05}} & \multicolumn{2}{l}{\rot{InternetAds\_10}} & \multicolumn{2}{l}{\rot{PageBlocks\_02}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &           0.678 &  0.183 &           0.722 &  0.100 &  \textbf{0.731} &  0.049 &  \textbf{0.649} &  0.034 &           0.688 &  0.088 &            0.65 &  0.053 &  \textbf{0.845} &  0.049 &           0.776 &  0.022 &           0.716 &  0.029 &  \textbf{0.850} &  0.022 \\
LOSEVM\_1       &           0.749 &  0.153 &           0.791 &  0.070 &           0.706 &  0.045 &           0.571 &  0.049 &           0.769 &  0.066 &           0.731 &  0.037 &           0.816 &  0.048 &           0.774 &  0.024 &           0.715 &  0.019 &           0.786 &  0.024 \\
LOSEVM\_5       &           0.804 &  0.151 &           0.837 &  0.072 &           0.713 &  0.043 &           0.615 &  0.035 &           0.781 &  0.061 &           0.781 &  0.042 &            0.81 &  0.047 &           0.778 &  0.025 &  \textbf{0.731} &  0.016 &           0.786 &  0.024 \\
LOSEVM\_10      &           0.808 &  0.153 &           0.839 &  0.071 &           0.715 &  0.045 &           0.618 &  0.035 &           0.797 &  0.072 &  \textbf{0.802} &  0.040 &            0.81 &  0.046 &            0.78 &  0.025 &            0.73 &  0.018 &           0.788 &  0.027 \\
LOSEVM\_20      &  \textbf{0.818} &  0.156 &  \textbf{0.848} &  0.074 &           0.725 &  0.038 &           0.621 &  0.035 &           0.791 &  0.077 &           0.801 &  0.039 &            0.81 &  0.046 &  \textbf{0.782} &  0.025 &  \textbf{0.731} &  0.017 &           0.787 &  0.025 \\
LOSEVM\_SVDD\_1  &            0.75 &  0.153 &            0.79 &  0.070 &           0.706 &  0.045 &            0.57 &  0.050 &           0.769 &  0.066 &           0.728 &  0.036 &           0.816 &  0.048 &           0.774 &  0.024 &           0.714 &  0.019 &           0.786 &  0.024 \\
LOSEVM\_SVDD\_5  &           0.806 &  0.149 &           0.826 &  0.080 &           0.717 &  0.042 &            0.62 &  0.033 &           0.782 &  0.062 &            0.78 &  0.042 &            0.81 &  0.047 &           0.777 &  0.025 &  \textbf{0.731} &  0.017 &           0.787 &  0.026 \\
LOSEVM\_SVDD\_10 &           0.807 &  0.151 &           0.826 &  0.081 &           0.718 &  0.042 &            0.62 &  0.035 &  \textbf{0.799} &  0.075 &           0.798 &  0.034 &            0.81 &  0.046 &            0.78 &  0.025 &  \textbf{0.731} &  0.018 &           0.787 &  0.025 \\
LOSEVM\_SVDD\_20 &           0.816 &  0.155 &  \textbf{0.848} &  0.070 &            0.73 &  0.042 &           0.623 &  0.033 &           0.792 &  0.078 &           0.801 &  0.037 &           0.809 &  0.046 &  \textbf{0.782} &  0.025 &  \textbf{0.731} &  0.017 &           0.787 &  0.025 \\
OCSVM          &           0.676 &  0.137 &           0.723 &  0.077 &           0.661 &  0.046 &           0.592 &  0.030 &           0.165 &  0.011 &           0.098 &  0.018 &           0.047 &  0.001 &           0.028 &  0.002 &           0.222 &  0.026 &           0.784 &  0.025 \\
SVDD           &           0.676 &  0.137 &           0.723 &  0.077 &           0.661 &  0.046 &           0.592 &  0.030 &           0.165 &  0.011 &           0.098 &  0.018 &           0.047 &  0.001 &           0.028 &  0.002 &           0.222 &  0.026 &           0.784 &  0.025 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{PageBlocks\_05}} & \multicolumn{2}{l}{\rot{Parkinson\_05}} & \multicolumn{2}{l}{\rot{Parkinson\_10}} & \multicolumn{2}{l}{\rot{Parkinson\_20}} & \multicolumn{2}{l}{\rot{PenDigits\_}} & \multicolumn{2}{l}{\rot{Pima\_02}} & \multicolumn{2}{l}{\rot{Pima\_05}} & \multicolumn{2}{l}{\rot{Pima\_10}} & \multicolumn{2}{l}{\rot{Pima\_20}} & \multicolumn{2}{l}{\rot{Shuttle\_}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &   std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &           0.768 &  0.027 &  \textbf{0.899} &  0.122 &  \textbf{0.929} &  0.029 &  \textbf{0.873} &  0.058 &  \textbf{0.936} &  0.02 &  \textbf{0.696} &  0.063 &  \textbf{0.692} &  0.050 &  \textbf{0.712} &  0.034 &  \textbf{0.702} &  0.019 &  \textbf{0.601} &  0.155 \\
LOSEVM\_1       &           0.788 &  0.015 &           0.774 &  0.303 &           0.712 &  0.109 &           0.636 &  0.073 &           0.806 &  0.00 &            0.64 &  0.116 &           0.636 &  0.045 &           0.618 &  0.027 &           0.592 &  0.039 &           0.553 &  0.145 \\
LOSEVM\_5       &           0.788 &  0.015 &           0.781 &  0.303 &           0.722 &  0.112 &           0.662 &  0.065 &           0.806 &  0.00 &           0.641 &  0.116 &           0.634 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &           0.553 &  0.144 \\
LOSEVM\_10      &           0.789 &  0.015 &           0.775 &  0.310 &            0.72 &  0.112 &           0.654 &  0.065 &           0.806 &  0.00 &           0.641 &  0.116 &           0.634 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &            0.56 &  0.135 \\
LOSEVM\_20      &           0.789 &  0.015 &           0.761 &  0.330 &           0.725 &  0.130 &           0.678 &  0.081 &           0.806 &  0.00 &           0.641 &  0.116 &           0.634 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &           0.558 &  0.138 \\
LOSEVM\_SVDD\_1  &           0.788 &  0.015 &           0.775 &  0.303 &           0.715 &  0.107 &           0.636 &  0.074 &           0.806 &  0.00 &           0.639 &  0.116 &           0.636 &  0.046 &           0.618 &  0.027 &           0.592 &  0.039 &           0.553 &  0.145 \\
LOSEVM\_SVDD\_5  &           0.789 &  0.014 &           0.776 &  0.300 &           0.724 &  0.111 &           0.665 &  0.062 &           0.806 &  0.00 &           0.641 &  0.117 &           0.634 &  0.044 &           0.618 &  0.027 &           0.593 &  0.040 &           0.552 &  0.145 \\
LOSEVM\_SVDD\_10 &           0.788 &  0.015 &           0.769 &  0.306 &            0.72 &  0.113 &           0.656 &  0.060 &           0.806 &  0.00 &           0.641 &  0.117 &           0.634 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &            0.56 &  0.134 \\
LOSEVM\_SVDD\_20 &  \textbf{0.790} &  0.014 &           0.764 &  0.306 &           0.735 &  0.130 &           0.725 &  0.095 &           0.806 &  0.00 &           0.641 &  0.117 &           0.634 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &           0.551 &  0.153 \\
OCSVM          &           0.786 &  0.015 &           0.706 &  0.242 &           0.689 &  0.140 &           0.597 &  0.048 &           0.806 &  0.00 &            0.64 &  0.116 &           0.633 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &           0.553 &  0.146 \\
SVDD           &           0.786 &  0.015 &           0.706 &  0.242 &           0.689 &  0.140 &           0.597 &  0.048 &           0.806 &  0.00 &            0.64 &  0.116 &           0.633 &  0.044 &           0.618 &  0.028 &           0.593 &  0.040 &           0.553 &  0.146 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{SpamBase\_02}} & \multicolumn{2}{l}{\rot{SpamBase\_05}} & \multicolumn{2}{l}{\rot{SpamBase\_10}} & \multicolumn{2}{l}{\rot{SpamBase\_20}} & \multicolumn{2}{l}{\rot{Stamps\_02}} & \multicolumn{2}{l}{\rot{Stamps\_05}} & \multicolumn{2}{l}{\rot{WBC\_}} & \multicolumn{2}{l}{\rot{WDBC\_}} & \multicolumn{2}{l}{\rot{Waveform\_}} & \multicolumn{2}{l}{\rot{Wilt\_02}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &  \textbf{0.775} &  0.038 &  \textbf{0.699} &  0.031 &  \textbf{0.623} &  0.031 &  \textbf{0.521} &  0.014 &  \textbf{0.866} &  0.079 &  \textbf{0.762} &  0.064 &  \textbf{0.975} &  0.010 &  \textbf{0.918} &  0.040 &  \textbf{0.699} &  0.036 &  \textbf{0.612} &  0.016 \\
LOSEVM\_1       &           0.619 &  0.043 &            0.59 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.697 &  0.098 &            0.61 &  0.083 &           0.927 &  0.056 &           0.883 &  0.049 &           0.577 &  0.032 &           0.433 &  0.019 \\
LOSEVM\_5       &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.675 &  0.088 &           0.593 &  0.064 &           0.928 &  0.062 &           0.885 &  0.049 &           0.587 &  0.023 &           0.433 &  0.019 \\
LOSEVM\_10      &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.675 &  0.088 &           0.594 &  0.065 &           0.929 &  0.060 &           0.889 &  0.045 &           0.587 &  0.023 &           0.433 &  0.019 \\
LOSEVM\_20      &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.675 &  0.088 &           0.594 &  0.065 &           0.929 &  0.061 &            0.89 &  0.044 &           0.587 &  0.023 &           0.433 &  0.019 \\
LOSEVM\_SVDD\_1  &           0.619 &  0.043 &            0.59 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.711 &  0.102 &           0.616 &  0.087 &           0.927 &  0.056 &           0.882 &  0.049 &           0.572 &  0.035 &           0.433 &  0.019 \\
LOSEVM\_SVDD\_5  &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.674 &  0.088 &           0.593 &  0.064 &           0.932 &  0.065 &           0.885 &  0.049 &           0.587 &  0.023 &           0.433 &  0.019 \\
LOSEVM\_SVDD\_10 &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.675 &  0.088 &           0.594 &  0.065 &           0.932 &  0.066 &           0.889 &  0.045 &           0.587 &  0.023 &           0.433 &  0.019 \\
LOSEVM\_SVDD\_20 &           0.619 &  0.043 &           0.591 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.675 &  0.088 &           0.593 &  0.065 &           0.932 &  0.066 &            0.89 &  0.045 &           0.587 &  0.023 &           0.433 &  0.018 \\
OCSVM          &           0.619 &  0.043 &            0.59 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.673 &  0.089 &           0.593 &  0.064 &           0.903 &  0.058 &           0.872 &  0.048 &           0.587 &  0.023 &           0.433 &  0.019 \\
SVDD           &           0.619 &  0.043 &            0.59 &  0.043 &           0.538 &  0.034 &           0.492 &  0.027 &           0.673 &  0.089 &           0.592 &  0.064 &           0.903 &  0.058 &           0.872 &  0.048 &           0.587 &  0.023 &           0.433 &  0.019 \\
\end{tabular}
\end{sidewaystable}








==> results_averprec.tex <==
\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}

datafile & \multicolumn{2}{l}{\rot{Annthyroid\_02}} & \multicolumn{2}{l}{\rot{Annthyroid\_05}} & \multicolumn{2}{l}{\rot{Arrhythmia\_02}} & \multicolumn{2}{l}{\rot{Arrhythmia\_05}} & \multicolumn{2}{l}{\rot{Arrhythmia\_10}} & \multicolumn{2}{l}{\rot{Arrhythmia\_20}} & \multicolumn{2}{l}{\rot{Cardiotocography\_02}} & \multicolumn{2}{l}{\rot{Cardiotocography\_05}} & \multicolumn{2}{l}{\rot{Cardiotocography\_10}} & \multicolumn{2}{l}{\rot{Cardiotocography\_20}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &                mean &    std &                mean &    std &                mean &    std &                mean &    std \\
\hline
KNN            &  \textbf{0.025} &  0.004 &  \textbf{0.041} &  0.003 &           0.278 &  0.167 &           0.347 &  0.120 &           0.416 &  0.090 &            0.43 &  0.066 &               0.151 &  0.041 &               0.154 &  0.024 &               0.111 &  0.021 &               0.042 &  0.009 \\
LOSEVM\_1       &           0.001 &  0.002 &          -0.001 &  0.001 &  \textbf{0.293} &  0.168 &  \textbf{0.381} &  0.140 &  \textbf{0.525} &  0.090 &  \textbf{0.550} &  0.066 &               0.123 &  0.042 &               0.155 &  0.034 &               0.187 &  0.049 &                0.26 &  0.076 \\
LOSEVM\_5       &           0.001 &  0.002 &            -0.0 &  0.001 &  \textbf{0.293} &  0.168 &           0.377 &  0.141 &           0.524 &  0.091 &  \textbf{0.550} &  0.066 &               0.128 &  0.033 &               0.169 &  0.040 &               0.204 &  0.028 &      \textbf{0.296} &  0.022 \\
LOSEVM\_10      &           0.002 &  0.002 &            -0.0 &  0.001 &  \textbf{0.293} &  0.168 &           0.377 &  0.141 &           0.523 &  0.091 &  \textbf{0.550} &  0.066 &               0.151 &  0.042 &               0.184 &  0.033 &                0.21 &  0.021 &               0.284 &  0.012 \\
LOSEVM\_20      &           0.002 &  0.002 &             0.0 &  0.001 &           0.292 &  0.168 &           0.377 &  0.141 &           0.523 &  0.091 &  \textbf{0.550} &  0.066 &      \textbf{0.153} &  0.045 &      \textbf{0.185} &  0.034 &      \textbf{0.214} &  0.021 &               0.288 &  0.010 \\
LOSEVM\_SVDD\_1  &           0.001 &  0.002 &          -0.001 &  0.001 &  \textbf{0.293} &  0.168 &  \textbf{0.381} &  0.140 &  \textbf{0.525} &  0.090 &  \textbf{0.550} &  0.066 &               0.123 &  0.042 &               0.154 &  0.033 &               0.186 &  0.050 &               0.259 &  0.075 \\
LOSEVM\_SVDD\_5  &           0.001 &  0.002 &            -0.0 &  0.001 &  \textbf{0.293} &  0.168 &           0.377 &  0.141 &           0.524 &  0.091 &  \textbf{0.550} &  0.066 &               0.135 &  0.038 &               0.166 &  0.038 &               0.206 &  0.026 &                0.29 &  0.018 \\
LOSEVM\_SVDD\_10 &           0.002 &  0.002 &            -0.0 &  0.001 &  \textbf{0.293} &  0.168 &           0.377 &  0.141 &           0.523 &  0.091 &  \textbf{0.550} &  0.066 &               0.148 &  0.040 &               0.182 &  0.033 &                0.21 &  0.023 &               0.284 &  0.010 \\
LOSEVM\_SVDD\_20 &           0.002 &  0.002 &             0.0 &  0.001 &           0.292 &  0.168 &           0.377 &  0.141 &           0.523 &  0.091 &  \textbf{0.550} &  0.066 &      \textbf{0.153} &  0.044 &               0.183 &  0.033 &      \textbf{0.214} &  0.023 &               0.287 &  0.013 \\
OCSVM          &           0.004 &  0.005 &           0.001 &  0.002 &           0.019 &  0.010 &           0.041 &  0.011 &            0.06 &  0.022 &           0.111 &  0.035 &               0.114 &  0.028 &               0.151 &  0.027 &               0.196 &  0.019 &               0.274 &  0.010 \\
SVDD           &           0.004 &  0.005 &           0.001 &  0.002 &           0.019 &  0.010 &           0.041 &  0.011 &            0.06 &  0.022 &           0.111 &  0.035 &               0.114 &  0.028 &               0.151 &  0.027 &               0.196 &  0.019 &               0.274 &  0.010 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{HeartDisease\_02}} & \multicolumn{2}{l}{\rot{HeartDisease\_05}} & \multicolumn{2}{l}{\rot{HeartDisease\_10}} & \multicolumn{2}{l}{\rot{HeartDisease\_20}} & \multicolumn{2}{l}{\rot{Hepatitis\_05}} & \multicolumn{2}{l}{\rot{Hepatitis\_10}} & \multicolumn{2}{l}{\rot{InternetAds\_02}} & \multicolumn{2}{l}{\rot{InternetAds\_05}} & \multicolumn{2}{l}{\rot{InternetAds\_10}} & \multicolumn{2}{l}{\rot{PageBlocks\_02}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &  \textbf{0.168} &  0.246 &           0.203 &  0.134 &           0.226 &  0.074 &           0.143 &  0.046 &           0.059 &  0.023 &           0.065 &  0.024 &           0.329 &  0.048 &           0.256 &  0.054 &  \textbf{0.208} &  0.026 &  \textbf{0.331} &  0.062 \\
LOSEVM\_1       &           0.072 &  0.064 &           0.194 &  0.110 &           0.196 &  0.074 &             0.1 &  0.070 &           0.087 &  0.031 &           0.093 &  0.023 &           0.423 &  0.060 &           0.325 &  0.052 &           0.183 &  0.023 &           0.231 &  0.028 \\
LOSEVM\_5       &           0.135 &  0.133 &           0.276 &  0.160 &           0.216 &  0.068 &           0.149 &  0.059 &           0.094 &  0.033 &           0.137 &  0.031 &           0.421 &  0.060 &           0.327 &  0.050 &  \textbf{0.208} &  0.020 &           0.222 &  0.030 \\
LOSEVM\_10      &           0.141 &  0.134 &           0.275 &  0.149 &           0.216 &  0.073 &           0.153 &  0.060 &           0.117 &  0.046 &  \textbf{0.167} &  0.051 &           0.422 &  0.058 &            0.33 &  0.049 &           0.206 &  0.023 &           0.209 &  0.033 \\
LOSEVM\_20      &           0.147 &  0.133 &  \textbf{0.308} &  0.162 &           0.227 &  0.065 &           0.156 &  0.057 &           0.111 &  0.060 &           0.163 &  0.045 &  \textbf{0.424} &  0.056 &           0.332 &  0.048 &           0.207 &  0.023 &           0.221 &  0.029 \\
LOSEVM\_SVDD\_1  &           0.073 &  0.064 &           0.194 &  0.110 &           0.196 &  0.074 &           0.099 &  0.070 &           0.087 &  0.031 &           0.091 &  0.022 &           0.423 &  0.060 &           0.325 &  0.052 &           0.183 &  0.022 &           0.231 &  0.029 \\
LOSEVM\_SVDD\_5  &           0.134 &  0.128 &           0.275 &  0.163 &           0.219 &  0.071 &           0.151 &  0.058 &           0.095 &  0.034 &           0.135 &  0.034 &           0.421 &  0.060 &           0.326 &  0.051 &           0.207 &  0.022 &           0.197 &  0.025 \\
LOSEVM\_SVDD\_10 &           0.139 &  0.134 &            0.27 &  0.161 &           0.223 &  0.073 &           0.154 &  0.060 &  \textbf{0.123} &  0.056 &           0.159 &  0.037 &           0.422 &  0.059 &            0.33 &  0.049 &           0.206 &  0.023 &           0.207 &  0.037 \\
LOSEVM\_SVDD\_20 &           0.143 &  0.131 &           0.304 &  0.158 &  \textbf{0.240} &  0.072 &  \textbf{0.161} &  0.056 &           0.114 &  0.060 &            0.16 &  0.044 &           0.422 &  0.058 &  \textbf{0.333} &  0.048 &           0.207 &  0.023 &           0.221 &  0.027 \\
OCSVM          &            0.06 &  0.106 &           0.064 &  0.028 &           0.104 &  0.041 &            0.08 &  0.033 &           -0.01 &  0.000 &          -0.039 &  0.001 &          -0.009 &  0.000 &          -0.025 &  0.000 &           -0.03 &  0.006 &           0.179 &  0.026 \\
SVDD           &            0.06 &  0.106 &           0.064 &  0.028 &           0.104 &  0.041 &            0.08 &  0.033 &           -0.01 &  0.000 &          -0.039 &  0.001 &          -0.009 &  0.000 &          -0.025 &  0.000 &          -0.031 &  0.006 &           0.179 &  0.029 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{PageBlocks\_05}} & \multicolumn{2}{l}{\rot{Parkinson\_05}} & \multicolumn{2}{l}{\rot{Parkinson\_10}} & \multicolumn{2}{l}{\rot{Parkinson\_20}} & \multicolumn{2}{l}{\rot{PenDigits\_}} & \multicolumn{2}{l}{\rot{Pima\_02}} & \multicolumn{2}{l}{\rot{Pima\_05}} & \multicolumn{2}{l}{\rot{Pima\_10}} & \multicolumn{2}{l}{\rot{Pima\_20}} & \multicolumn{2}{l}{\rot{Shuttle\_}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &           0.285 &  0.022 &  \textbf{0.516} &  0.319 &  \textbf{0.571} &  0.167 &  \textbf{0.631} &  0.101 &  \textbf{0.045} &  0.015 &            0.04 &  0.020 &            0.07 &  0.028 &  \textbf{0.126} &  0.044 &  \textbf{0.195} &  0.023 &  \textbf{0.081} &  0.064 \\
LOSEVM\_1       &  \textbf{0.300} &  0.033 &           0.445 &  0.349 &           0.328 &  0.145 &           0.404 &  0.106 &           0.003 &  0.000 &  \textbf{0.049} &  0.031 &  \textbf{0.071} &  0.035 &           0.074 &  0.030 &           0.111 &  0.024 &           0.018 &  0.015 \\
LOSEVM\_5       &           0.272 &  0.057 &           0.484 &  0.365 &           0.353 &  0.141 &           0.423 &  0.107 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &            0.08 &  0.033 &           0.114 &  0.024 &           0.024 &  0.023 \\
LOSEVM\_10      &            0.27 &  0.046 &           0.494 &  0.363 &           0.358 &  0.138 &           0.416 &  0.107 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &            0.08 &  0.033 &           0.115 &  0.023 &           0.024 &  0.024 \\
LOSEVM\_20      &           0.267 &  0.036 &           0.476 &  0.369 &           0.348 &  0.157 &           0.448 &  0.143 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &            0.08 &  0.033 &           0.115 &  0.023 &           0.029 &  0.028 \\
LOSEVM\_SVDD\_1  &  \textbf{0.300} &  0.033 &           0.446 &  0.348 &           0.334 &  0.135 &           0.404 &  0.106 &           0.003 &  0.000 &  \textbf{0.049} &  0.031 &  \textbf{0.071} &  0.035 &           0.074 &  0.030 &           0.111 &  0.024 &           0.018 &  0.015 \\
LOSEVM\_SVDD\_5  &           0.285 &  0.041 &            0.47 &  0.372 &           0.363 &  0.136 &           0.425 &  0.101 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &           0.081 &  0.034 &           0.114 &  0.024 &           0.026 &  0.027 \\
LOSEVM\_SVDD\_10 &           0.273 &  0.049 &           0.471 &  0.369 &           0.371 &  0.133 &           0.414 &  0.098 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &            0.08 &  0.033 &           0.115 &  0.023 &           0.025 &  0.025 \\
LOSEVM\_SVDD\_20 &           0.268 &  0.049 &           0.429 &  0.360 &           0.381 &  0.200 &           0.517 &  0.114 &           0.003 &  0.000 &           0.048 &  0.029 &           0.068 &  0.031 &            0.08 &  0.033 &           0.115 &  0.023 &           0.026 &  0.025 \\
OCSVM          &           0.265 &  0.033 &           0.139 &  0.167 &           0.162 &  0.113 &           0.149 &  0.056 &           0.003 &  0.000 &           0.035 &  0.035 &           0.062 &  0.038 &           0.072 &  0.029 &           0.105 &  0.027 &           0.025 &  0.022 \\
SVDD           &           0.266 &  0.033 &           0.139 &  0.167 &           0.162 &  0.113 &           0.149 &  0.056 &           0.003 &  0.000 &           0.035 &  0.036 &           0.062 &  0.038 &           0.072 &  0.029 &           0.105 &  0.027 &           0.027 &  0.024 \\
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\centering
\begin{tabular}{llrlrlrlrlrlrlrlrlrlr}
datafile & \multicolumn{2}{l}{\rot{SpamBase\_02}} & \multicolumn{2}{l}{\rot{SpamBase\_05}} & \multicolumn{2}{l}{\rot{SpamBase\_10}} & \multicolumn{2}{l}{\rot{SpamBase\_20}} & \multicolumn{2}{l}{\rot{Stamps\_02}} & \multicolumn{2}{l}{\rot{Stamps\_05}} & \multicolumn{2}{l}{\rot{WBC\_}} & \multicolumn{2}{l}{\rot{WDBC\_}} & \multicolumn{2}{l}{\rot{Waveform\_}} & \multicolumn{2}{l}{\rot{Wilt\_02}} \\
algorithm &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std &            mean &    std \\
\hline
KNN            &  \textbf{0.077} &  0.027 &  \textbf{0.088} &  0.013 &  \textbf{0.088} &  0.018 &  \textbf{0.049} &  0.011 &  \textbf{0.125} &  0.058 &  \textbf{0.123} &  0.048 &           0.733 &  0.098 &           0.259 &  0.076 &  \textbf{0.071} &  0.019 &  \textbf{0.004} &  0.001 \\
LOSEVM\_1       &           0.033 &  0.016 &           0.036 &  0.010 &           0.028 &  0.012 &           0.006 &  0.014 &           0.053 &  0.033 &           0.041 &  0.030 &           0.826 &  0.089 &           0.318 &  0.104 &           0.012 &  0.006 &          -0.002 &  0.001 \\
LOSEVM\_5       &           0.042 &  0.018 &           0.041 &  0.012 &           0.031 &  0.012 &           0.008 &  0.014 &           0.063 &  0.045 &           0.041 &  0.025 &           0.838 &  0.121 &           0.337 &  0.118 &           0.014 &  0.005 &          -0.002 &  0.001 \\
LOSEVM\_10      &           0.042 &  0.018 &           0.041 &  0.012 &           0.031 &  0.012 &           0.008 &  0.014 &            0.06 &  0.045 &           0.042 &  0.024 &           0.844 &  0.123 &           0.347 &  0.127 &           0.014 &  0.005 &          -0.002 &  0.001 \\
LOSEVM\_20      &           0.041 &  0.018 &           0.041 &  0.012 &           0.031 &  0.012 &           0.008 &  0.014 &            0.06 &  0.045 &            0.04 &  0.025 &           0.843 &  0.125 &  \textbf{0.349} &  0.126 &           0.014 &  0.005 &          -0.002 &  0.001 \\
LOSEVM\_SVDD\_1  &           0.033 &  0.016 &           0.036 &  0.010 &           0.028 &  0.012 &           0.006 &  0.014 &           0.055 &  0.034 &           0.041 &  0.030 &           0.826 &  0.089 &           0.318 &  0.104 &           0.011 &  0.006 &          -0.002 &  0.001 \\
LOSEVM\_SVDD\_5  &           0.042 &  0.018 &           0.041 &  0.012 &           0.031 &  0.011 &           0.008 &  0.014 &           0.063 &  0.044 &           0.041 &  0.026 &  \textbf{0.848} &  0.123 &           0.336 &  0.116 &           0.014 &  0.005 &          -0.002 &  0.001 \\
LOSEVM\_SVDD\_10 &           0.042 &  0.018 &           0.041 &  0.012 &           0.031 &  0.012 &           0.008 &  0.014 &            0.06 &  0.045 &           0.043 &  0.027 &  \textbf{0.848} &  0.133 &           0.348 &  0.129 &           0.014 &  0.005 &          -0.002 &  0.001 \\
LOSEVM\_SVDD\_20 &           0.042 &  0.018 &           0.041 &  0.012 &           0.031 &  0.012 &           0.008 &  0.014 &            0.06 &  0.045 &           0.038 &  0.024 &           0.845 &  0.136 &  \textbf{0.349} &  0.128 &           0.014 &  0.005 &          -0.002 &  0.001 \\
OCSVM          &           0.029 &  0.019 &           0.029 &  0.011 &           0.023 &  0.012 &           0.004 &  0.014 &            0.04 &  0.030 &           0.035 &  0.023 &           0.417 &  0.119 &           0.178 &  0.055 &           0.016 &  0.007 &          -0.002 &  0.001 \\
SVDD           &           0.029 &  0.019 &           0.029 &  0.011 &           0.023 &  0.012 &           0.004 &  0.014 &            0.04 &  0.030 &           0.034 &  0.023 &           0.417 &  0.119 &           0.178 &  0.055 &           0.016 &  0.007 &          -0.002 &  0.001 \\
\end{tabular}
\end{sidewaystable}







